Robust Blind Deconvolution via Mirror Descent

We revisit the Blind Deconvolution problem with a focus on understanding its robustness and convergence properties. Provable robustness to noise and other perturbations is receiving recent interest in vision, from obtaining immunity to adversarial attacks to assessing and describing failure modes of algorithms in mission critical applications. Further, many blind deconvolution methods based on deep architectures internally make use of or optimize the basic formulation, so a clearer understanding of how this sub-module behaves, when it can be solved, and what noise injection it can tolerate is a first order requirement. We derive new insights into the theoretical underpinnings of blind deconvolution. The algorithm that emerges has nice convergence guarantees and is provably robust in a sense we formalize in the paper. Interestingly, these technical results play out very well in practice, where on standard datasets our algorithm yields results competitive with or superior to the state of the art. Keywords: blind deconvolution, robust continuous optimization

==> abstract.tex <==
\begin{abstract}
%	Large strides have recently been made in sharp image recovery given only a blurred input. This process of blind deconvolution has been solved in a variety of contexts, each of which brings a new perspective to the problem, and with it a new type of model. Often, these models are context-specific, and fail to generalize well to other imaging domains. Additionally, many modern methods, some based on the recent successes of deep learning models, have been shown to be particularly sensitive to input noise in training data. Motivated by these problems, we propose a generalized image deblurring method, PRIDA, which, we show to be provably robust and convergent. Applying our method to standard deblurring datasets, we find that our method outperforms recent methods in the presence of noise, and recovers quality sharp images when applied to real-world images.
We revisit a classical problem in computer vision and image analysis called as Blind Deconvolution. In this problem, given a blurred image, the goal is to recover the associated sharp image and the blur kernel simultaneously. Although the literature in this area is mature, the algorithmic underpinnings of the problem is still not fully understood and is being actively researched. In this work, we propose an efficient algorithm, PRIDA, using ideas from Convex Geometry. Theoretically, we analyze both the \emph{convergence} and \emph{robustness} properties of PRIDA. Empirically, we perform an extensive set of experiments to validate our theoretical findings on two standard datasets. Our results (see Figure \ref{fig:teaser}) show that PRIDA beats the state-of-the-art algorithms under wide range of noise conditions implying that the algorithm is effective in practice.
\end{abstract}
